Online monitoring for safe pedestrian-vehicle interactions

As autonomous systems begin to operate amongst humans, methods for safe interaction must be investigated. We consider an example of a small autonomous vehicle in a pedestrian zone that must safely maneuver around people in a free-form fashion. We investigate two key questions: How can we effectively integrate pedestrian intent estimation into our autonomous stack. Can we develop an online monitoring framework to give formal guarantees on the safety of such human-robot interactions. We present a pedestrian intent estimation framework that can accurately predict future pedestrian trajectories given multiple possible goal locations. We integrate this into a reachability-based online monitoring scheme that formally assesses the safety of these interactions with nearly real-time performance (approximately 0.3 seconds). These techniques are integrated on a test vehicle with a complete in-house autonomous stack, demonstrating effective and safe interaction in real-world experiments.

==> 05_Experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{EXPERIMENTS}
Section on experiment setup and the scenarios we are using

\sayan{These are the end-to-end experiments.}

[kt:] I vote we kill this section and merge it with the results section

==> dm.tex <==
Input: $\tau = \{\langle p_i, t_i \rangle\}, r_s, \{\ell_i\}$
        $p_c = \mathit{intersect}(\tau,\{\ell_i\})$
        if $p_c = \bot$ then output $\mathit{go}$
        else
                $t_c$ time corresp. to $p_c$ in $\tau$
                $B = B(p_c,r_s)$
                $\tau_v = \mathit{simulate}(x,v,t_0,\{\ell_i\})$
                $[t_1,t_2] = \mathit{interTime}(\tau_v,B)$
                if $t_c \in [t_1, t_2]$ 
                        then output $\mathit{brake}$
                else if $t_c \in [t_1-t_s, t_2+t_s]$
                        then output $\mathit{slow}$
                else output $\mathit{go}$
